Learning an Adaptive Model for Extreme Low-light Raw Image Processing

Low-light images suffer from severe noise and low illumination. Current deep learning models that are trained with real-world images have excellent noise reduction, but a ratio parameter must be chosen manually to complete the enhancement pipeline. In this work, we propose an adaptive low-light raw image enhancement network to avoid parameter-handcrafting and to improve image quality. The proposed method can be divided into two sub-models: Brightness Prediction (BP) and Exposure Shifting (ES). The former is designed to control the brightness of the resulting image by estimating a guideline exposure time $t_1$. The latter learns to approximate an exposure-shifting operator $ES$, converting a low-light image with real exposure time $t_0$ to a noise-free image with guideline exposure time $t_1$. Additionally, structural similarity (SSIM) loss and Image Enhancement Vector (IEV) are introduced to promote image quality, and a new Campus Image Dataset (CID) is proposed to overcome the limitations of the existing datasets and to supervise the training of the proposed model. Using the proposed model, we can achieve high-quality low-light image enhancement from a single raw image. In quantitative tests, it is shown that the proposed method has the lowest Noise Level Estimation (NLE) score compared with the state-of-the-art low-light algorithms, suggesting a superior denoising performance. Furthermore, those tests illustrate that the proposed method is able to adaptively control the global image brightness according to the content of the image scene. Lastly, the potential application in video processing is briefly discussed.

==> compare_imgdpi.tex <==

\begin{figure}[!t]
  \centering
  \includegraphics[width=3.5in]{bshift}
  \caption{The shift of average brightness and brightness coefficient of variation (CV) 
  within each group. Each Group contain 3--6 images captured in a brust with different 
  exposure time, e.g. Fig.\ref{exp}. In both test set and training set, an increase in brightness 
  and reduction in CV is observed. Note that the CV decreased considerably, indicating the 
  highly uniformed brightness for images within each group after enhancement.}
  \label{brightnessshift}
  \end{figure}

  \begin{figure*}[h!t] %#强制单栏排版
    \centering %#居中
    %\begin{minipage}[b]{1\linewidth} %#整体划分一个0.93倍页面宽度的页面
    \subfloat[original]{
      \begin{minipage}[b]{0.1292\linewidth} %#继续划分子页面 每个宽度0.12倍总宽度
        \centering
        %#依次读取每张图片  宽度或者高度可以自定义
        %#这里的几张图片是纵向排列的
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/0_orig__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/orig__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/0_orig__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/orig__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/0_orig__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/orig__.jpg}
      \end{minipage}
    }
    \hfill
     \subfloat[MSR]{
      \begin{minipage}[b]{0.1292\linewidth}
        \centering
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/10_MSR__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/MSR__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/10_MSR__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/MSR__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/10_MSR__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/MSR__.jpg}
      \end{minipage}
    }
    \hfill
      \subfloat[MSR+BM3D]{
      \begin{minipage}[b]{0.1292\linewidth}
        \centering
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/1_MSRBM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/MSRBM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/1_MSRBM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/MSRBM3D__.jpg}\vspace{4pt}      
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/1_MSRBM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/MSRBM3D__.jpg}
      \end{minipage}
    }
    \hfill
      \subfloat[LIME+BM3D]{
      \begin{minipage}[b]{0.1292\linewidth}
        \centering
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/2_LIME_BM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/LIME_BM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/2_LIME_BM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/LIME_BM3D__.jpg}\vspace{4pt}      
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/2_LIME_BM3D__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/LIME_BM3D__.jpg}
      \end{minipage}
    }
    \hfill
      \subfloat[R-Net+BM3D]{
      \begin{minipage}[b]{0.1292\linewidth}
        \centering
  
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/3_RetinexNET__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/01tools/RetinexNET__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/3_RetinexNET__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/02lab/RetinexNET__.jpg}\vspace{4pt}      
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/3_RetinexNET__.jpg}\vspace{4pt}
        \includegraphicsdpi{600}{width=\textwidth}{img/03text/RetinexNET__.jpg}
      \end{minipage}
    }
    \hfill
    \subfloat[SID]{
    \begin{minipage}[b]{0.1292\linewidth}
      \centering
  
      \includegraphicsdpi{600}{width=\textwidth}{img/01tools/4_SID__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/01tools/SID__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/02lab/4_SID__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/02lab/SID__.jpg}\vspace{4pt}    
      \includegraphicsdpi{600}{width=\textwidth}{img/03text/4_SID__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/03text/SID__.jpg}
    \end{minipage}
    }
    \hfill
    \subfloat[our method]{
    \begin{minipage}[b]{0.1292\linewidth}
      \centering
      \includegraphicsdpi{600}{width=\textwidth}{img/01tools/5_ours__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/01tools/ours__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/02lab/5_ours__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/02lab/ours__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/03text/5_ours__.jpg}\vspace{4pt}
      \includegraphicsdpi{600}{width=\textwidth}{img/03text/ours__.jpg}
    \end{minipage}
    }
  
    %\end{minipage}
    %\vfill
    \caption{The results using different methods on CID test images.
    From (a) to (g), they are the original low-light images and the results of multiscale Retinex (MSR), MSR with BM3D,
    illumination map estimation based (LIME), LIME with BM3D, deep Retinex decomposition (R-net), R-net with BM3D, 
    learning-to-see-in-the-dark (SID) model and ours respectively.
    }
  \label{compare}
  \end{figure*}


  % From the left column to the right column, 
  %   they are original low-light images, 
  %   multiscale Retinex (MSR), MSR implementing BM3D,
  %   illumination map estimation based (LIME), LIME implementing BM3D,
  %   deep Retinex decomposition (R-Net), R-Net implementing BM3D, 
  %   learning-to-see-in-the-dark (SID) model and our method.

==> exp_imgdpi.tex <==




\begin{figure*}
  \centering
  \begin{tabular}{ccccc}
  
  
    \rotatebox[origin=c]{90}{low-light image}
    &
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/JPEG_2019_09_19_20_52_01_725.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/JPEG_2019_09_19_20_52_01_855.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/JPEG_2019_09_19_20_52_02_042.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/JPEG_2019_09_19_20_52_02_097.jpg}
    \end{minipage}   
     
    \\   %换列
  
    \rotatebox[origin=c]{90}{our method}
    &
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/1_20.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/1_50.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/1_80.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/04road/1_100.jpg}
    \end{minipage}   
    \\   %换列
  
  
    (a) & 1/20 seconds & 1/50 seconds & 1/80 seconds  & 1/100 seconds  
     
     \\
    
    \rotatebox[origin=c]{90}{low-light image}
    &
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/05stick/JPEG_2019_09_18_11_08_00_533.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/05stick/JPEG_2019_09_18_11_08_00_664.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/05stick/JPEG_2019_09_18_11_08_00_787.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
    \includegraphicsdpi{600}{width=\textwidth}{img/05stick/JPEG_2019_09_18_11_08_00_842.jpg}
    \end{minipage}   
  
    \\   %换列
  
    \rotatebox[origin=c]{90}{our method}
    &
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/05stick/RAW_2019_09_18_11_08_00_521dngenhanced.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/05stick/RAW_2019_09_18_11_08_00_626dngenhanced.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
    \includegraphicsdpi{600}{width=\textwidth}{img/05stick/RAW_2019_09_18_11_08_00_753dngenhanced.jpg}
    \end{minipage}   
    &   %换行
    \begin{minipage}{0.2\textwidth}
      \includegraphicsdpi{600}{width=\textwidth}{img/05stick/RAW_2019_09_18_11_08_00_805dngenhanced.jpg}
    \end{minipage}   
    \\   %换列
  
   
     (b) & 1/20 seconds & 1/60 seconds & 1/125 seconds  & 1/250 seconds  
  
  \end{tabular}
  \caption{The results of using our method to enhance multiple images 
  in a same scene but captured with diverse exposure time. 
  For the second image group, The exposure time $t_0$ of the last image in the sequence is only 8\% of that of the first, yet the network compensates for this difference, 
  keeping the brightness of each image in the scene approximately uniform.}
  \label{exp}
  \end{figure*}
